Benchmarking Graph Neural Networks

In the last few years, graph neural networks (GNNs) have become the standard toolkit for analyzing and learning from data on graphs. This emerging field has witnessed an extensive growth of promising techniques that have been applied with success to computer science, mathematics, biology, physics and chemistry. But for any successful field to become mainstream and reliable, benchmarks must be developed to quantify progress. This led us in March 2020 to release a benchmark framework that i) comprises of a diverse collection of mathematical and real-world graphs, ii) enables fair model comparison with the same parameter budget to identify key architectures, iii) has an open-source, easy-to-use and reproducible code infrastructure, and iv) is flexible for researchers to experiment with new theoretical ideas. As of December 2022, the GitHub repository has reached 2,000 stars and 380 forks, which demonstrates the utility of the proposed open-source framework through the wide usage by the GNN community. In this paper, we present an updated version of our benchmark with a concise presentation of the aforementioned framework characteristics, an additional medium-sized molecular dataset AQSOL, similar to the popular ZINC, but with a real-world measured chemical target, and discuss how this framework can be leveraged to explore new GNN designs and insights. As a proof of value of our benchmark, we study the case of graph positional encoding (PE) in GNNs, which was introduced with this benchmark and has since spurred interest of exploring more powerful PE for Transformers and GNNs in a robust experimental setting.

==> all_results.tex <==


% % [OLD] TABLE WITH PE = ABS VAL(EIGNVEC)
% \begin{table}[t!]
%     \centering
%     \caption{
%     Benchmarking results for MP-GCNs and WL-GNNs across 7 medium-scale graph classification/regression and node/link prediction datasets.
%     Results are averaged over 4 runs with 4 different seeds. \best{Red}: the best model, \good{Violet}: good models. 
%     }
%     \vspace{3pt}
%     \scalebox{0.5}{
%     \begin{tabular}{rr|ccccc|ccccc}
%         \toprule
%         & & \multicolumn{10}{c}{\textbf{NODE CLASSIFICATION}} \\
%         & & \multicolumn{5}{c}{\textbf{PATTERN}} & \multicolumn{5}{c}{\textbf{CLUSTER}}\\
%         \textbf{Model} & \textbf{$L$} & \textbf{\#Param} & \textbf{Test Acc.$\pm$s.d.} & \textbf{Train Acc.$\pm$s.d.} & \textbf{\#Epoch} & \textbf{Epoch/Total} & \textbf{\#Param} & \textbf{Test Acc.$\pm$s.d.} & \textbf{Train Acc.$\pm$s.d.} & \textbf{\#Epoch} & \textbf{Epoch/Total} \\
%         \midrule
%         \midrule
%         MLP & 4 & 105263 & 50.519$\pm$0.000 & 50.487$\pm$0.014 & 42.25 & 8.95s/0.11hr & 106015 & 20.973$\pm$0.004 & 20.938$\pm$0.002 & 42.25 & 5.83s/0.07hr\\
%         \midrule
%         GCN & 4 & 100923 & 63.880$\pm$0.074 & 65.126$\pm$0.135 & 105.00 & 118.85s/3.51hr & 101655 & 53.445$\pm$2.029 & 54.041$\pm$2.197 & 70.00 & 65.72s/1.30hr\\
%         & 16 & 500823 & 71.892$\pm$0.334 & 78.409$\pm$1.592 & 81.50 & 492.19s/11.31hr & 501687 & 68.498$\pm$0.976 & 71.729$\pm$2.212 & 79.75 & 270.28s/6.08hr\\
%         GraphSage & 4 & 101739 & 50.516$\pm$0.001 & 50.473$\pm$0.014 & 43.75 & 93.41s/1.17hr & 102187 & 50.454$\pm$0.145 & 54.374$\pm$0.203 & 64.00 & 53.56s/0.97hr\\
%         & 16 & 502842 & 50.492$\pm$0.001 & 50.487$\pm$0.005 & 46.50 & 391.19s/5.19hr & 503350 & 63.844$\pm$0.110 & 86.710$\pm$0.167 & 57.75 & 225.61s/3.70hr\\
%         \midrule
%         % MoNet & 4 & 103775 & {85.287$\pm$0.113} & 85.304$\pm$0.134 & 43.00 & 996.95s/12.41hr & 104227 & 57.508$\pm$0.660 & 57.826$\pm$0.693 & 63.75 & 692.79s/12.18hr\\
%         % OPTIMIZED MoNet below
%         MoNet & 4 & 103775 & \good{85.482$\pm$0.037} & 85.569$\pm$0.044 & 89.75 & 35.71s/0.90hr & 104227 & 58.064$\pm$0.131 & 58.454$\pm$0.183 & 76.25 & 24.29s/0.52hr\\
%         % & 16 & 511487 & \good{85.417$\pm$0.203} & 85.483$\pm$0.193 & 40.00 & 1068.77s/12.37hr & 511999 & 65.830$\pm$1.108 & 66.996$\pm$1.152 & 66.00 & 652.34s/12.28hr\\
%         % OPTIMIZED MoNet below
%         & 16 & 511487 & \good{85.582$\pm$0.038} & 85.720$\pm$0.068 & 81.75 & 68.49s/1.58hr & 511999 & 66.407$\pm$0.540 & 67.727$\pm$0.649 & 77.75 & 47.82s/1.05hr\\
%         GAT & 4 & 109936 & 75.824$\pm$1.823 & 77.883$\pm$1.632 & 96.00 & 20.92s/0.57hr & 110700 & 57.732$\pm$0.323 & 58.331$\pm$0.342 & 67.25 & 14.17s/0.27hr\\
%         & 16 & 526990 & 78.271$\pm$0.186 & 90.212$\pm$0.476 & 53.50 & 50.33s/0.77hr & 527874 & \good{70.587$\pm$0.447} & 76.074$\pm$1.362 & 73.50 & 35.94s/0.75hr\\
%         GatedGCN & 4 & 104003 & 84.480$\pm$0.122 & 84.474$\pm$0.155 & 78.75 & 139.01s/3.09hr & 104355 & 60.404$\pm$0.419 & 61.618$\pm$0.536 & 94.50 & 79.97s/2.13hr\\
%         & 16 & 502223 & \good{85.568$\pm$0.088} & 86.007$\pm$0.123 & 65.25 & 644.71s/11.91hr & 502615 & \best{73.840$\pm$0.326} & 87.880$\pm$0.908 & 60.00 & 400.07s/6.81hr\\
%         GatedGCN-PE & 16 & 505421 & \best{86.363$\pm$0.127} & 86.810$\pm$0.126 & 60.00 & 647.95s/11.09hr & 503473 & \best{74.088$\pm$0.344} & 90.252$\pm$1.048 & 56.50 & 400.34s/6.45hr \\
%         \midrule
%         GIN & 4 & 100884 & \good{85.590$\pm$0.011} & 85.852$\pm$0.030 & 93.00 & 15.24s/0.40hr & 103544 & 58.384$\pm$0.236 & 59.480$\pm$0.337 & 74.75 & 10.71s/0.23hr\\
%         & 16 & 508574 & 85.387$\pm$0.136 & 85.664$\pm$0.116 & 86.75 & 25.14s/0.62hr & 517570 & 64.716$\pm$1.553 & 65.973$\pm$1.816 & 80.75 & 20.67s/0.47hr\\
%         RingGNN & 2 & 105206 & \good{86.245$\pm$0.013} & 86.118$\pm$0.034 & 75.00 & 573.37s/12.17hr & 104746 & 42.418$\pm$20.063 & 42.520$\pm$20.212 & 74.50 & 428.24s/8.79hr\\
%         & 2 & 504766 & \good{86.244$\pm$0.025} & 86.105$\pm$0.021 & 72.00 & 595.97s/12.15hr & 524202 & 22.340$\pm$0.000 & 22.304$\pm$0.000 & 43.25 & 501.84s/6.22hr\\
%         & 8 & 505749 & \textrm{Diverged} & \textrm{Diverged} & \textrm{Diverged} & \textrm{Diverged} & 514380 & \textrm{Diverged} & \textrm{Diverged} & \textrm{Diverged} & \textrm{Diverged}\\
%         3WLGNN & 3 & 103572 & \good{85.661$\pm$0.353} & 85.608$\pm$0.337 & 95.00 & 304.79s/7.88hr & 105552 & 57.130$\pm$6.539 & 57.404$\pm$6.597 & 116.00 & 219.51s/6.52hr\\
%         & 3 & 502872 & \good{85.341$\pm$0.207} & 85.270$\pm$0.198 & 81.75 & 424.23s/9.56hr & 507252 & 55.489$\pm$7.863 & 55.736$\pm$8.024 & 66.00 & 319.98s/5.79hr \\
%         & 8 & 581716 & \textrm{Diverged} & \textrm{Diverged} & \textrm{Diverged} & \textrm{Diverged} & 586788 & \textrm{Diverged} & \textrm{Diverged} & \textrm{Diverged} & \textrm{Diverged}\\
%         \midrule
%         \midrule
%         & & \multicolumn{10}{c}{\textbf{GRAPH CLASSIFICATION}} \\
%         & & \multicolumn{5}{c}{\textbf{MNIST}} & \multicolumn{5}{c}{\textbf{CIFAR10}}\\
%         \textbf{Model} & \textbf{$L$} & \textbf{\#Param} & \textbf{Test Acc.$\pm$s.d.} & \textbf{Train Acc.$\pm$s.d.} & \textbf{\#Epoch} & \textbf{Epoch/Total} & \textbf{\#Param} & \textbf{Test Acc.$\pm$s.d.} & \textbf{Train Acc.$\pm$s.d.} & \textbf{\#Epoch} & \textbf{Epoch/Total} \\
%         \midrule
%         \midrule
%         MLP & 4 & 104044 & 95.340$\pm$0.138 & 97.432$\pm$0.470 & 232.25 & 22.74s/1.48hr & 104380 & 56.340$\pm$0.181 & 65.113$\pm$1.685 & 185.25 & 29.48s/1.53hr\\
%         \midrule
%         GCN & 4 & 101365 & 90.705$\pm$0.218 & 97.196$\pm$0.223 & 127.50 & 83.41s/2.99hr & 101657 & 55.710$\pm$0.381 & 69.523$\pm$1.948 & 142.50 & 109.70s/4.39hr\\
%         GraphSage & 4 & 104337 & \best{97.312$\pm$0.097} & 100.000$\pm$0.000 & 98.25 & 113.12s/3.13hr & 104517 & \good{65.767$\pm$0.308} & 99.719$\pm$0.062 & 93.50 & 124.61s/3.29hr\\
%         \midrule
%         % MoNet & 4 & 104049 & 88.507$\pm$1.414 & 90.895$\pm$1.910 & 57.75 & 750.10s/12.28hr & 104229 & 49.462$\pm$1.386 & 52.671$\pm$1.991 & 42.50 & 1031.36s/12.42hr\\
%         % OPTIMIZED MoNet below
%         MoNet & 4 & 104049 & 90.805$\pm$0.032 & 96.609$\pm$0.440 & 146.25 & 93.19s/3.82hr & 104229 & 54.655$\pm$0.518 & 65.911$\pm$2.515 & 141.50 & 97.13s/3.85hr\\
%         GAT & 4 & 110400 & 95.535$\pm$0.205 & 99.994$\pm$0.008 & 104.75 & 42.26s/1.25hr & 110704 & 64.223$\pm$0.455 & 89.114$\pm$0.499 & 103.75 & 55.27s/1.62hr\\
%         GatedGCN & 4 & 104217 & \best{97.340$\pm$0.143} & 100.000$\pm$0.000 & 96.25 & 128.79s/3.50hr & 104357 & \best{67.312$\pm$0.311} & 94.553$\pm$1.018 & 97.00 & 154.15s/4.22hr\\
%         %& GatedGCN-E & 4 & 104217 & \best{97.350$\pm$0.098} & 100.000$\pm$0.000 & 96.00 & 133.47s/3.61hr \\
%         \midrule
%         GIN & 4 & 105434 & \good{96.485$\pm$0.252} & 100.000$\pm$0.000 & 128.00 & 39.22s/1.41hr & 105654 & 55.255$\pm$1.527 & 79.412$\pm$9.700 & 141.50 & 52.12s/2.07hr\\
%         RingGNN & 2 & 105398 & 11.350$\pm$0.000 & 11.235$\pm$0.000 & 14.00 & 2945.69s/12.77hr & 105165 & 19.300$\pm$16.108 & 19.556$\pm$16.397 & 13.50 & 3112.96s/13.00hr\\
%         & 2 & 505182 & 91.860$\pm$0.449 & 92.169$\pm$0.505 & 16.25 & 2575.99s/12.63hr & 504949 & 39.165$\pm$17.114 & 40.209$\pm$17.790 & 13.75 & 2998.24s/12.60hr \\
%         & 8 & 506357 & Diverged & Diverged & Diverged & Diverged & 510439 & Diverged & Diverged & Diverged & Diverged\\
%         3WLGNN & 3 & 108024 & 95.075$\pm$0.961 & 95.830$\pm$1.338 & 27.75 & 1523.20s/12.40hr & 108516 & 59.175$\pm$1.593 & 63.751$\pm$2.697 & 28.50 & 1506.29s/12.60hr \\
%         & 3 & 501690 & 95.002$\pm$0.419 & 95.692$\pm$0.677 & 26.25 & 1608.73s/12.42hr & 502770 & 58.043$\pm$2.512 & 61.574$\pm$3.575 & 20.00 & 2091.22s/12.55hr\\
%         & 8 & 500816 & Diverged & Diverged & Diverged & Diverged & 501584 & Diverged & Diverged & Diverged & Diverged \\
%         \midrule
%         \midrule
%         & & \multicolumn{10}{c}{\textbf{LINK PREDICTION}} \\
%         & & \multicolumn{5}{c}{\textbf{TSP}} & \multicolumn{5}{c}{\textbf{COLLAB}}\\
%         \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{$L$}} & \multirow{2}{*}{\textbf{\#Param}} & \multirow{2}{*}{\textbf{Test F1$\pm$s.d.}} & \multirow{2}{*}{\textbf{Train F1$\pm$s.d.}} & \multirow{2}{*}{\textbf{\#Epoch}} & \multirow{2}{*}{\textbf{Epoch/Total}} & \textbf{\#Param} & \multirow{2}{*}{\textbf{Test Hits$\pm$s.d.}} & \multirow{2}{*}{\textbf{Train Hits$\pm$s.d.}} & \multirow{2}{*}{\textbf{\#Epoch}} & \multirow{2}{*}{\textbf{Epoch/Total}} \\
%          & & & & & & & $\mathbf{(\textit{L}=3)}$ & & & & \\
%         \midrule
%         \midrule
%         MLP & 4 & 96956 & 0.544$\pm$0.001 & 0.544$\pm$0.001 & 164.25 & 50.15s/2.31hr & 39441 & 20.350$\pm$2.168 & 29.807$\pm$3.360 & 147.50 & 2.09s/0.09hr \\
%         \midrule
%         GCN & 4 & 95702 & 0.630$\pm$0.001 & 0.631$\pm$0.001 & 261.00 & 152.89s/11.15hr & 40479 & 50.422$\pm$1.131 & 92.112$\pm$0.991 & 122.50 & 351.05s/12.04hr \\
%         GraphSage & 4 & 99263 & 0.665$\pm$0.003 & 0.669$\pm$0.003 & 266.00 & 157.26s/11.68hr & 39856 & \good{51.618$\pm$0.690} & 99.949$\pm$0.052 & 152.75 & 277.93s/11.87hr \\
%         \midrule
%         % MoNet & 4 & 99007 & 0.561$\pm$0.018 & 0.561$\pm$0.018 & 27.50 & 1573.25s/12.66hr & 39751 & 36.144$\pm$2.191 & 61.156$\pm$3.973 & 167.50 & 26.69s/1.26hr \\
%         % OPTIMIZED MoNet below
%         MoNet & 4 & 99007 & 0.641$\pm$0.002 & 0.643$\pm$0.002 & 282.00 & 84.46s/6.65hr & 39751 & 36.144$\pm$2.191 & 61.156$\pm$3.973 & 167.50 & 26.69s/1.26hr \\
%         GAT & 4 & 96182 & 0.671$\pm$0.002 & 0.673$\pm$0.002 & 328.25 & 68.23s/6.25hr & 42637 & \good{51.501$\pm$0.962} & 97.851$\pm$1.114 & 157.00 & 18.12s/0.80hr \\
%         GatedGCN & 4 & 97858 & \good{0.791$\pm$0.003} & 0.793$\pm$0.003 & 159.00 & 218.20s/9.72hr & 40965 & \best{52.816$\pm$1.303} & 96.537$\pm$1.614 & 95.00 & 451.92s/12.05hr \\
%         GatedGCN-PE & & \multicolumn{5}{c|}{-} & 42769 & \good{52.018$\pm$1.178} & 96.208$\pm$1.833 & 94.50 & 452.34s/12.05hr \\
%         GatedGCN-E & 4 & 97858 & \good{0.808$\pm$0.003} & 0.811$\pm$0.003 & 197.00 & 218.51s/12.04hr & 40965 & 49.212$\pm$1.560 & 88.747$\pm$1.058 & 95.00 & 451.21s/12.03hr \\
%         GatedGCN-E & 16 & 500770 & \best{0.838$\pm$0.002} & 0.850$\pm$0.001 & 53.00 & 807.23s/12.17hr & \multicolumn{5}{c}{-} \\
%         \midrule
%         GIN & 4 & 99002 & 0.656$\pm$0.003 & 0.660$\pm$0.003 & 273.50 & 72.73s/5.56hr & 39544 & 41.730$\pm$2.284 & 70.555$\pm$4.444 & 140.25 & 8.66s/0.34hr \\
%         RingGNN & 2 & 106862 & 0.643$\pm$0.024 & 0.644$\pm$0.024 & 2.00 & 17850.52s/17.19hr & - & OOM & \multicolumn{3}{c}{ 
%         \multirow{6}{2in}{RingGNN and 3WLGNN rely on dense tensors which leads to \textbf{OOM} on both GPU and CPU memory. 
%         }} \\
%         & 2 & 507938 & 0.704$\pm$0.003 & 0.705$\pm$0.003 & 3.00 & 12835.53s/16.08hr & - & OOM & \\
%         & 8 & 506564 & Diverged & Diverged & Diverged & Diverged & - & OOM & \\
%         3WLGNN & 3 & 106366 & 0.694$\pm$0.073 & 0.695$\pm$0.073 & 2.00 & 17468.81s/16.59hr & - & OOM & \\
%         & 3 & 506681 & 0.288$\pm$0.311 & 0.290$\pm$0.312 & 2.00 & 17190.17s/16.51hr & - & OOM &\\
%         % & 3 & 503964 & 0.000$\pm$0.000 & 0.000$\pm$0.000 & 1.00 & 30809.80s/21.18hr \\
%         & 8 & 508832 & OOM & OOM & OOM & OOM & - & OOM & \\
%         \midrule
%         $k$-NN Heuristic & & $k=$2 & \multicolumn{4}{l|}{Test F1: 0.693} \\
%         Matrix Fact. & 0 & \multicolumn{5}{c|}{-} & 60546561 & 44.206$\pm$0.452 & 100.000$\pm$0.000 & 254.33 & 2.66s/0.21hr \\
%         \midrule
%         \midrule
%         & & \multicolumn{5}{c|}{\textbf{GRAPH REGRESSION -- ZINC}} &
%         \multicolumn{5}{c}{
%         \multirow{26}{4.2in}{
%         $\!\!$\textbf{Evaluation Metrics:} (higher is better, except for ZINC)\\
%         \vspace{-0.1cm}
%         \begin{itemize}[leftmargin=*]
%             \item CLUSTER, PATTERN use weighted accuracy w.r.t. the class sizes. \vspace{-0.05cm}
%             \item MNIST, CIFAR10 use multi-label classification accuracy. \vspace{-0.05cm}
%             \item TSP uses binary F1 score for the positive edges. \vspace{-0.05cm}
%             \item COLLAB uses Hits@50 via the evaluator provided by OGB~\cite{hu2020ogb}. \vspace{-0.05cm}
%             \item ZINC uses mean absolute regression error.% (lower is better).
%         \end{itemize}
%         \vspace{0.05cm}
%         \textbf{Notation:}\\
%         \vspace{-0.1cm}
%         \begin{itemize}[leftmargin=*]
%             \item Models with the suffix \textbf{-E} use input edge features to initialize edge representations (ZINC: bond type, TSP: Euclidean distance, COLLAB: collaboration frequency and year).\vspace{-0.05cm}
%             \item Models with the suffix \textbf{-PE} use Laplacian Eigenvectors as node positional encodings, with dimension 8 for ZINC and 40 for others.\vspace{-0.05cm}
%             \item Results denoted by \textbf{Diverged} indicate unstable and divergent runs across all 4 seeds and initial learning rate values $\{10^{-3}, 10^{-4}, 10^{-5}\}$.\vspace{-0.05cm}
%             \item Results denoted by \textbf{OOM} indicate runs which throw out of memory errors on our hardware configuration.\vspace{-0.05cm}
%         \end{itemize}
%         \vspace{0.05cm}
%         \textbf{Extended training:}\\
%         \vspace{-0.1cm}
%         \begin{itemize}[leftmargin=*]
%             \item For TSP, RingGNN/3WLGNN with 100K parameters achieved 0.733$\pm$0.020 and 0.649$\pm$0.051 respectively after 48hr of training.
%         \end{itemize}
%         } } \\
%         \textbf{Model} & \textbf{$L$} & \textbf{\#Param} & \textbf{Test MAE$\pm$s.d.} & \textbf{Train MAE$\pm$s.d.} & \textbf{\#Epoch} & \textbf{Epoch/Total} & \\
%         \cline{1-7}
%         \cline{1-7}
%         MLP & 4 & 108975 & 0.706$\pm$0.006 & 0.644$\pm$0.005 & 116.75 & 1.01s/0.03hr \\
%         % & 16 & 505225 & 0.711$\pm$0.001 & 0.654$\pm$0.003 & 104.25 & 1.50s/0.04hr \\
%         % \midrule
%         \cline{1-7}
%         GCN & 4 & 103077 & 0.459$\pm$0.006 & 0.343$\pm$0.011 & 196.25 & 2.89s/0.16hr & \\
%          & 16 & 505079 & 0.367$\pm$0.011 & 0.128$\pm$0.019 & 197.00 & 12.78s/0.71hr & \\
%         GraphSage & 4 & 94977 & 0.468$\pm$0.003 & 0.251$\pm$0.004 & 147.25 & 3.74s/0.15hr & \\
%          & 16 & 505341 & 0.398$\pm$0.002 & 0.081$\pm$0.009 & 145.50 & 16.61s/0.68hr & \\
%         % \midrule
%         \cline{1-7}
%         % MoNet & 4 & 106002 & 0.388$\pm$0.008 & 0.295$\pm$0.019 & 154.75 & 12.33s/0.54hr \\
%         %  & 16 & 504013 & 0.294$\pm$0.011 & 0.115$\pm$0.015 & 152.00 & 20.74s/0.88hr \\
%         % OPTIMIZED MoNet below
%         MoNet & 4 & 106002 & 0.397$\pm$0.010 & 0.318$\pm$0.016 & 188.25 & 1.97s/0.10hr \\
%         & 16 & 504013 & 0.292$\pm$0.006 & 0.093$\pm$0.014 & 171.75 & 10.82s/0.52hr\\
%         GAT & 4 & 102385 & 0.475$\pm$0.007 & 0.317$\pm$0.006 & 137.50 & 2.93s/0.11hr & \\
%          & 16 & 531345 & 0.384$\pm$0.007 & 0.067$\pm$0.004 & 144.00 & 12.98s/0.53hr & \\
%         GatedGCN & 4 & 105735 & 0.435$\pm$0.011 & 0.287$\pm$0.014 & 173.50 & 5.76s/0.28hr & \\
%         GatedGCN-E & 4 & 105875 & 0.375$\pm$0.003 & 0.236$\pm$0.007 & 194.75 & 5.37s/0.29hr & \\
%          & 16 & 504309 & \good{0.282$\pm$0.015} & 0.074$\pm$0.016 & 166.75 & 20.50s/0.96hr & \\
%         GatedGCN-E-PE & 16 & 505011 & \best{0.214$\pm$0.006} & 0.033$\pm$0.012 & 167.00 & 20.74s/0.98hr \\
%         % \midrule
%         \cline{1-7}
%         GIN & 4 & 103079 & 0.387$\pm$0.015 & 0.319$\pm$0.015 & 153.25 & 2.29s/0.10hr \\
%          & 16 & 509549 & 0.526$\pm$0.051 & 0.444$\pm$0.039 & 147.00 & 10.22s/0.42hr \\
%         RingGNN & 2 & 97978 & 0.512$\pm$0.023 & 0.383$\pm$0.020 & 90.25 & 327.65s/8.32hr  \\
%         RingGNN-E & 2 & 104403 & 0.363$\pm$0.026 & 0.243$\pm$0.025 & 95.00 & 366.29s/9.76hr \\
%          & 2 & 527283 & 0.353$\pm$0.019 & 0.236$\pm$0.019 & 79.75 & 293.94s/6.63hr \\
%           & 8 & 510305 & Diverged & Diverged & Diverged & Diverged \\
%         3WLGNN & 3 & 102150 & 0.407$\pm$0.028 & 0.272$\pm$0.037 & 111.25 & 286.23s/8.88hr  \\
%         3WLGNN-E & 3 & 103098 & \good{0.256$\pm$0.054} & 0.140$\pm$0.044 & 117.25 & 334.69s/10.90hr \\
%          & 3 & 507603 & 0.303$\pm$0.068 & 0.173$\pm$0.041 & 120.25 & 329.49s/11.08hr \\
%          & 8 & 582824 & 0.303$\pm$0.057 & 0.246$\pm$0.043 & 52.50 & 811.27s/12.15hr \\
%         \bottomrule
%     \end{tabular}
%     }
%     \label{tab:results}
% \end{table}



% [NEW] TABLES WITH PE = RAND SIGN(EIGNVEC)
\begin{table}[t!]
    \centering
    \caption{
    Benchmarking results for MP-GCNs and WL-GNNs across 7 medium-scale graph classification/regression and node/link prediction datasets.
    Results are averaged over 4 runs with 4 different seeds. \best{Red}: the best model, \good{Violet}: good models. 
    }
    \vspace{3pt}
    \scalebox{0.5}{
    \begin{tabular}{rr|ccccc|ccccc}
        \toprule
        & & \multicolumn{10}{c}{\textbf{NODE CLASSIFICATION}} \\
        & & \multicolumn{5}{c}{\textbf{PATTERN}} & \multicolumn{5}{c}{\textbf{CLUSTER}}\\
        \textbf{Model} & \textbf{$L$} & \textbf{\#Param} & \textbf{Test Acc.$\pm$s.d.} & \textbf{Train Acc.$\pm$s.d.} & \textbf{\#Epoch} & \textbf{Epoch/Total} & \textbf{\#Param} & \textbf{Test Acc.$\pm$s.d.} & \textbf{Train Acc.$\pm$s.d.} & \textbf{\#Epoch} & \textbf{Epoch/Total} \\
        \midrule
        \midrule
        MLP & 4 & 105263 & 50.519$\pm$0.000 & 50.487$\pm$0.014 & 42.25 & 8.95s/0.11hr & 106015 & 20.973$\pm$0.004 & 20.938$\pm$0.002 & 42.25 & 5.83s/0.07hr\\
        \midrule
        GCN & 4 & 100923 & 63.880$\pm$0.074 & 65.126$\pm$0.135 & 105.00 & 118.85s/3.51hr & 101655 & 53.445$\pm$2.029 & 54.041$\pm$2.197 & 70.00 & 65.72s/1.30hr\\
        & 16 & 500823 & 71.892$\pm$0.334 & 78.409$\pm$1.592 & 81.50 & 492.19s/11.31hr & 501687 & 68.498$\pm$0.976 & 71.729$\pm$2.212 & 79.75 & 270.28s/6.08hr\\
        GraphSage & 4 & 101739 & 50.516$\pm$0.001 & 50.473$\pm$0.014 & 43.75 & 93.41s/1.17hr & 102187 & 50.454$\pm$0.145 & 54.374$\pm$0.203 & 64.00 & 53.56s/0.97hr\\
        & 16 & 502842 & 50.492$\pm$0.001 & 50.487$\pm$0.005 & 46.50 & 391.19s/5.19hr & 503350 & 63.844$\pm$0.110 & 86.710$\pm$0.167 & 57.75 & 225.61s/3.70hr\\
        \midrule
        % MoNet & 4 & 103775 & {85.287$\pm$0.113} & 85.304$\pm$0.134 & 43.00 & 996.95s/12.41hr & 104227 & 57.508$\pm$0.660 & 57.826$\pm$0.693 & 63.75 & 692.79s/12.18hr\\
        % OPTIMIZED MoNet below
        MoNet & 4 & 103775 & \good{85.482$\pm$0.037} & 85.569$\pm$0.044 & 89.75 & 35.71s/0.90hr & 104227 & 58.064$\pm$0.131 & 58.454$\pm$0.183 & 76.25 & 24.29s/0.52hr\\
        % & 16 & 511487 & \good{85.417$\pm$0.203} & 85.483$\pm$0.193 & 40.00 & 1068.77s/12.37hr & 511999 & 65.830$\pm$1.108 & 66.996$\pm$1.152 & 66.00 & 652.34s/12.28hr\\
        % OPTIMIZED MoNet below
        & 16 & 511487 & \good{85.582$\pm$0.038} & 85.720$\pm$0.068 & 81.75 & 68.49s/1.58hr & 511999 & 66.407$\pm$0.540 & 67.727$\pm$0.649 & 77.75 & 47.82s/1.05hr\\
        GAT & 4 & 109936 & 75.824$\pm$1.823 & 77.883$\pm$1.632 & 96.00 & 20.92s/0.57hr & 110700 & 57.732$\pm$0.323 & 58.331$\pm$0.342 & 67.25 & 14.17s/0.27hr\\
        & 16 & 526990 & 78.271$\pm$0.186 & 90.212$\pm$0.476 & 53.50 & 50.33s/0.77hr & 527874 & \good{70.587$\pm$0.447} & 76.074$\pm$1.362 & 73.50 & 35.94s/0.75hr\\
        GatedGCN & 4 & 104003 & 84.480$\pm$0.122 & 84.474$\pm$0.155 & 78.75 & 139.01s/3.09hr & 104355 & 60.404$\pm$0.419 & 61.618$\pm$0.536 & 94.50 & 79.97s/2.13hr\\
        & 16 & 502223 & \good{85.568$\pm$0.088} & 86.007$\pm$0.123 & 65.25 & 644.71s/11.91hr & 502615 & \good{73.840$\pm$0.326} & 87.880$\pm$0.908 & 60.00 & 400.07s/6.81hr\\
        GatedGCN-PE & 16 & 502457 & \best{86.508$\pm$0.085} & 86.801$\pm$0.133 & 65.75 & 647.94s/12.08hr & 504253 & \best{76.082$\pm$0.196} & 88.919$\pm$0.720 & 57.75 & 399.66s/6.58hr \\
        \midrule
        GIN & 4 & 100884 & \good{85.590$\pm$0.011} & 85.852$\pm$0.030 & 93.00 & 15.24s/0.40hr & 103544 & 58.384$\pm$0.236 & 59.480$\pm$0.337 & 74.75 & 10.71s/0.23hr\\
        & 16 & 508574 & 85.387$\pm$0.136 & 85.664$\pm$0.116 & 86.75 & 25.14s/0.62hr & 517570 & 64.716$\pm$1.553 & 65.973$\pm$1.816 & 80.75 & 20.67s/0.47hr\\
        RingGNN & 2 & 105206 & \good{86.245$\pm$0.013} & 86.118$\pm$0.034 & 75.00 & 573.37s/12.17hr & 104746 & 42.418$\pm$20.063 & 42.520$\pm$20.212 & 74.50 & 428.24s/8.79hr\\
        & 2 & 504766 & \good{86.244$\pm$0.025} & 86.105$\pm$0.021 & 72.00 & 595.97s/12.15hr & 524202 & 22.340$\pm$0.000 & 22.304$\pm$0.000 & 43.25 & 501.84s/6.22hr\\
        & 8 & 505749 & \textrm{Diverged} & \textrm{Diverged} & \textrm{Diverged} & \textrm{Diverged} & 514380 & \textrm{Diverged} & \textrm{Diverged} & \textrm{Diverged} & \textrm{Diverged}\\
        3WLGNN & 3 & 103572 & \good{85.661$\pm$0.353} & 85.608$\pm$0.337 & 95.00 & 304.79s/7.88hr & 105552 & 57.130$\pm$6.539 & 57.404$\pm$6.597 & 116.00 & 219.51s/6.52hr\\
        & 3 & 502872 & \good{85.341$\pm$0.207} & 85.270$\pm$0.198 & 81.75 & 424.23s/9.56hr & 507252 & 55.489$\pm$7.863 & 55.736$\pm$8.024 & 66.00 & 319.98s/5.79hr \\
        & 8 & 581716 & \textrm{Diverged} & \textrm{Diverged} & \textrm{Diverged} & \textrm{Diverged} & 586788 & \textrm{Diverged} & \textrm{Diverged} & \textrm{Diverged} & \textrm{Diverged}\\
        \midrule
        \midrule
        & & \multicolumn{10}{c}{\textbf{GRAPH CLASSIFICATION}} \\
        & & \multicolumn{5}{c}{\textbf{MNIST}} & \multicolumn{5}{c}{\textbf{CIFAR10}}\\
        \textbf{Model} & \textbf{$L$} & \textbf{\#Param} & \textbf{Test Acc.$\pm$s.d.} & \textbf{Train Acc.$\pm$s.d.} & \textbf{\#Epoch} & \textbf{Epoch/Total} & \textbf{\#Param} & \textbf{Test Acc.$\pm$s.d.} & \textbf{Train Acc.$\pm$s.d.} & \textbf{\#Epoch} & \textbf{Epoch/Total} \\
        \midrule
        \midrule
        MLP & 4 & 104044 & 95.340$\pm$0.138 & 97.432$\pm$0.470 & 232.25 & 22.74s/1.48hr & 104380 & 56.340$\pm$0.181 & 65.113$\pm$1.685 & 185.25 & 29.48s/1.53hr\\
        \midrule
        GCN & 4 & 101365 & 90.705$\pm$0.218 & 97.196$\pm$0.223 & 127.50 & 83.41s/2.99hr & 101657 & 55.710$\pm$0.381 & 69.523$\pm$1.948 & 142.50 & 109.70s/4.39hr\\
        GraphSage & 4 & 104337 & \best{97.312$\pm$0.097} & 100.000$\pm$0.000 & 98.25 & 113.12s/3.13hr & 104517 & \good{65.767$\pm$0.308} & 99.719$\pm$0.062 & 93.50 & 124.61s/3.29hr\\
        \midrule
        % MoNet & 4 & 104049 & 88.507$\pm$1.414 & 90.895$\pm$1.910 & 57.75 & 750.10s/12.28hr & 104229 & 49.462$\pm$1.386 & 52.671$\pm$1.991 & 42.50 & 1031.36s/12.42hr\\
        % OPTIMIZED MoNet below
        MoNet & 4 & 104049 & 90.805$\pm$0.032 & 96.609$\pm$0.440 & 146.25 & 93.19s/3.82hr & 104229 & 54.655$\pm$0.518 & 65.911$\pm$2.515 & 141.50 & 97.13s/3.85hr\\
        GAT & 4 & 110400 & 95.535$\pm$0.205 & 99.994$\pm$0.008 & 104.75 & 42.26s/1.25hr & 110704 & 64.223$\pm$0.455 & 89.114$\pm$0.499 & 103.75 & 55.27s/1.62hr\\
        GatedGCN & 4 & 104217 & \best{97.340$\pm$0.143} & 100.000$\pm$0.000 & 96.25 & 128.79s/3.50hr & 104357 & \best{67.312$\pm$0.311} & 94.553$\pm$1.018 & 97.00 & 154.15s/4.22hr\\
        %& GatedGCN-E & 4 & 104217 & \best{97.350$\pm$0.098} & 100.000$\pm$0.000 & 96.00 & 133.47s/3.61hr \\
        \midrule
        GIN & 4 & 105434 & \good{96.485$\pm$0.252} & 100.000$\pm$0.000 & 128.00 & 39.22s/1.41hr & 105654 & 55.255$\pm$1.527 & 79.412$\pm$9.700 & 141.50 & 52.12s/2.07hr\\
        RingGNN & 2 & 105398 & 11.350$\pm$0.000 & 11.235$\pm$0.000 & 14.00 & 2945.69s/12.77hr & 105165 & 19.300$\pm$16.108 & 19.556$\pm$16.397 & 13.50 & 3112.96s/13.00hr\\
        & 2 & 505182 & 91.860$\pm$0.449 & 92.169$\pm$0.505 & 16.25 & 2575.99s/12.63hr & 504949 & 39.165$\pm$17.114 & 40.209$\pm$17.790 & 13.75 & 2998.24s/12.60hr \\
        & 8 & 506357 & Diverged & Diverged & Diverged & Diverged & 510439 & Diverged & Diverged & Diverged & Diverged\\
        3WLGNN & 3 & 108024 & 95.075$\pm$0.961 & 95.830$\pm$1.338 & 27.75 & 1523.20s/12.40hr & 108516 & 59.175$\pm$1.593 & 63.751$\pm$2.697 & 28.50 & 1506.29s/12.60hr \\
        & 3 & 501690 & 95.002$\pm$0.419 & 95.692$\pm$0.677 & 26.25 & 1608.73s/12.42hr & 502770 & 58.043$\pm$2.512 & 61.574$\pm$3.575 & 20.00 & 2091.22s/12.55hr\\
        & 8 & 500816 & Diverged & Diverged & Diverged & Diverged & 501584 & Diverged & Diverged & Diverged & Diverged \\
        \midrule
        \midrule
        & & \multicolumn{10}{c}{\textbf{LINK PREDICTION}} \\
        & & \multicolumn{5}{c}{\textbf{TSP}} & \multicolumn{5}{c}{\textbf{COLLAB}}\\
        \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{$L$}} & \multirow{2}{*}{\textbf{\#Param}} & \multirow{2}{*}{\textbf{Test F1$\pm$s.d.}} & \multirow{2}{*}{\textbf{Train F1$\pm$s.d.}} & \multirow{2}{*}{\textbf{\#Epoch}} & \multirow{2}{*}{\textbf{Epoch/Total}} & \textbf{\#Param} & \multirow{2}{*}{\textbf{Test Hits$\pm$s.d.}} & \multirow{2}{*}{\textbf{Train Hits$\pm$s.d.}} & \multirow{2}{*}{\textbf{\#Epoch}} & \multirow{2}{*}{\textbf{Epoch/Total}} \\
         & & & & & & & $\mathbf{(\textit{L}=3)}$ & & & & \\
        \midrule
        \midrule
        MLP & 4 & 96956 & 0.544$\pm$0.001 & 0.544$\pm$0.001 & 164.25 & 50.15s/2.31hr & 39441 & 20.350$\pm$2.168 & 29.807$\pm$3.360 & 147.50 & 2.09s/0.09hr \\
        \midrule
        GCN & 4 & 95702 & 0.630$\pm$0.001 & 0.631$\pm$0.001 & 261.00 & 152.89s/11.15hr & 40479 & 50.422$\pm$1.131 & 92.112$\pm$0.991 & 122.50 & 351.05s/12.04hr \\
        GraphSage & 4 & 99263 & 0.665$\pm$0.003 & 0.669$\pm$0.003 & 266.00 & 157.26s/11.68hr & 39856 & \good{51.618$\pm$0.690} & 99.949$\pm$0.052 & 152.75 & 277.93s/11.87hr \\
        \midrule
        % MoNet & 4 & 99007 & 0.561$\pm$0.018 & 0.561$\pm$0.018 & 27.50 & 1573.25s/12.66hr & 39751 & 36.144$\pm$2.191 & 61.156$\pm$3.973 & 167.50 & 26.69s/1.26hr \\
        % OPTIMIZED MoNet below
        MoNet & 4 & 99007 & 0.641$\pm$0.002 & 0.643$\pm$0.002 & 282.00 & 84.46s/6.65hr & 39751 & 36.144$\pm$2.191 & 61.156$\pm$3.973 & 167.50 & 26.69s/1.26hr \\
        GAT & 4 & 96182 & 0.671$\pm$0.002 & 0.673$\pm$0.002 & 328.25 & 68.23s/6.25hr & 42637 & \good{51.501$\pm$0.962} & 97.851$\pm$1.114 & 157.00 & 18.12s/0.80hr \\
        GatedGCN & 4 & 97858 & \good{0.791$\pm$0.003} & 0.793$\pm$0.003 & 159.00 & 218.20s/9.72hr & 40965 & \good{52.635$\pm$1.168} & 96.103$\pm$1.876 & 95.00 & 453.47s/12.09hr \\
        GatedGCN-PE & & \multicolumn{5}{c|}{-} & 41889 & \best{52.849$\pm$1.345} & 96.165$\pm$0.453 & 94.75 & 452.75s/12.08hr \\
        GatedGCN-E & 4 & 97858 & \good{0.808$\pm$0.003} & 0.811$\pm$0.003 & 197.00 & 218.51s/12.04hr & 40965 & 49.212$\pm$1.560 & 88.747$\pm$1.058 & 95.00 & 451.21s/12.03hr \\
        GatedGCN-E & 16 & 500770 & \best{0.838$\pm$0.002} & 0.850$\pm$0.001 & 53.00 & 807.23s/12.17hr & \multicolumn{5}{c}{-} \\
        \midrule
        GIN & 4 & 99002 & 0.656$\pm$0.003 & 0.660$\pm$0.003 & 273.50 & 72.73s/5.56hr & 39544 & 41.730$\pm$2.284 & 70.555$\pm$4.444 & 140.25 & 8.66s/0.34hr \\
        RingGNN & 2 & 106862 & 0.643$\pm$0.024 & 0.644$\pm$0.024 & 2.00 & 17850.52s/17.19hr & - & OOM & \multicolumn{3}{c}{ 
        \multirow{6}{2in}{RingGNN and 3WLGNN rely on dense tensors which leads to \textbf{OOM} on both GPU and CPU memory. 
        }} \\
        & 2 & 507938 & 0.704$\pm$0.003 & 0.705$\pm$0.003 & 3.00 & 12835.53s/16.08hr & - & OOM & \\
        & 8 & 506564 & Diverged & Diverged & Diverged & Diverged & - & OOM & \\
        3WLGNN & 3 & 106366 & 0.694$\pm$0.073 & 0.695$\pm$0.073 & 2.00 & 17468.81s/16.59hr & - & OOM & \\
        & 3 & 506681 & 0.288$\pm$0.311 & 0.290$\pm$0.312 & 2.00 & 17190.17s/16.51hr & - & OOM &\\
        % & 3 & 503964 & 0.000$\pm$0.000 & 0.000$\pm$0.000 & 1.00 & 30809.80s/21.18hr \\
        & 8 & 508832 & OOM & OOM & OOM & OOM & - & OOM & \\
        \midrule
        $k$-NN Heuristic & & $k=$2 & \multicolumn{4}{l|}{Test F1: 0.693} \\
        Matrix Fact. & 0 & \multicolumn{5}{c|}{-} & 60546561 & 44.206$\pm$0.452 & 100.000$\pm$0.000 & 254.33 & 2.66s/0.21hr \\
        \midrule
        \midrule
        & & \multicolumn{5}{c|}{\textbf{GRAPH REGRESSION -- ZINC}} &
        \multicolumn{5}{c}{
        \multirow{26}{4.2in}{
        $\!\!$\textbf{Evaluation Metrics:} (higher is better, except for ZINC)\\
        \vspace{-0.1cm}
        \begin{itemize}[leftmargin=*]
            \item CLUSTER, PATTERN use weighted accuracy w.r.t. the class sizes. \vspace{-0.05cm}
            \item MNIST, CIFAR10 use multi-label classification accuracy. \vspace{-0.05cm}
            \item TSP uses binary F1 score for the positive edges. \vspace{-0.05cm}
            \item COLLAB uses Hits@50 via the evaluator provided by OGB~\cite{hu2020ogb}. \vspace{-0.05cm}
            \item ZINC uses mean absolute regression error.% (lower is better).
        \end{itemize}
        \vspace{0.05cm}
        \textbf{Notation:}\\
        \vspace{-0.1cm}
        \begin{itemize}[leftmargin=*]
            \item Models with the suffix \textbf{-E} use input edge features to initialize edge representations (ZINC: bond type, TSP: Euclidean distance, COLLAB: collaboration frequency and year).\vspace{-0.05cm}
            \item Models with the suffix \textbf{-PE} use Laplacian Eigenvectors as node positional encodings, with dimension 8 for ZINC, 2 for PATTERN and 20 for others.\vspace{-0.05cm}
            \item Results denoted by \textbf{Diverged} indicate unstable and divergent runs across all 4 seeds and initial learning rate values $\{10^{-3}, 10^{-4}, 10^{-5}\}$.\vspace{-0.05cm}
            \item Results denoted by \textbf{OOM} indicate runs which throw out of memory errors on our hardware configuration.\vspace{-0.05cm}
        \end{itemize}
        \vspace{0.05cm}
        \textbf{Extended training:}\\
        \vspace{-0.1cm}
        \begin{itemize}[leftmargin=*]
            \item For TSP, RingGNN/3WLGNN with 100K parameters achieved 0.733$\pm$0.020 and 0.649$\pm$0.051 respectively after 48hr of training.
        \end{itemize}
        } } \\
        \textbf{Model} & \textbf{$L$} & \textbf{\#Param} & \textbf{Test MAE$\pm$s.d.} & \textbf{Train MAE$\pm$s.d.} & \textbf{\#Epoch} & \textbf{Epoch/Total} & \\
        \cline{1-7}
        \cline{1-7}
        MLP & 4 & 108975 & 0.706$\pm$0.006 & 0.644$\pm$0.005 & 116.75 & 1.01s/0.03hr \\
        % & 16 & 505225 & 0.711$\pm$0.001 & 0.654$\pm$0.003 & 104.25 & 1.50s/0.04hr \\
        % \midrule
        \cline{1-7}
        GCN & 4 & 103077 & 0.459$\pm$0.006 & 0.343$\pm$0.011 & 196.25 & 2.89s/0.16hr & \\
         & 16 & 505079 & 0.367$\pm$0.011 & 0.128$\pm$0.019 & 197.00 & 12.78s/0.71hr & \\
        GraphSage & 4 & 94977 & 0.468$\pm$0.003 & 0.251$\pm$0.004 & 147.25 & 3.74s/0.15hr & \\
         & 16 & 505341 & 0.398$\pm$0.002 & 0.081$\pm$0.009 & 145.50 & 16.61s/0.68hr & \\
        % \midrule
        \cline{1-7}
        % MoNet & 4 & 106002 & 0.388$\pm$0.008 & 0.295$\pm$0.019 & 154.75 & 12.33s/0.54hr \\
        %  & 16 & 504013 & 0.294$\pm$0.011 & 0.115$\pm$0.015 & 152.00 & 20.74s/0.88hr \\
        % OPTIMIZED MoNet below
        MoNet & 4 & 106002 & 0.397$\pm$0.010 & 0.318$\pm$0.016 & 188.25 & 1.97s/0.10hr \\
        & 16 & 504013 & 0.292$\pm$0.006 & 0.093$\pm$0.014 & 171.75 & 10.82s/0.52hr\\
        GAT & 4 & 102385 & 0.475$\pm$0.007 & 0.317$\pm$0.006 & 137.50 & 2.93s/0.11hr & \\
         & 16 & 531345 & 0.384$\pm$0.007 & 0.067$\pm$0.004 & 144.00 & 12.98s/0.53hr & \\
        GatedGCN & 4 & 105735 & 0.435$\pm$0.011 & 0.287$\pm$0.014 & 173.50 & 5.76s/0.28hr & \\
        GatedGCN-E & 4 & 105875 & 0.375$\pm$0.003 & 0.236$\pm$0.007 & 194.75 & 5.37s/0.29hr & \\
         & 16 & 504309 & \good{0.282$\pm$0.015} & 0.074$\pm$0.016 & 166.75 & 20.50s/0.96hr & \\
        GatedGCN-E-PE & 16 & 505011 & \best{0.214$\pm$0.013} & 0.067$\pm$0.019 & 185.00 & 10.70s/0.56hr \\
        % \midrule
        \cline{1-7}
        GIN & 4 & 103079 & 0.387$\pm$0.015 & 0.319$\pm$0.015 & 153.25 & 2.29s/0.10hr \\
         & 16 & 509549 & 0.526$\pm$0.051 & 0.444$\pm$0.039 & 147.00 & 10.22s/0.42hr \\
        RingGNN & 2 & 97978 & 0.512$\pm$0.023 & 0.383$\pm$0.020 & 90.25 & 327.65s/8.32hr  \\
        RingGNN-E & 2 & 104403 & 0.363$\pm$0.026 & 0.243$\pm$0.025 & 95.00 & 366.29s/9.76hr \\
         & 2 & 527283 & 0.353$\pm$0.019 & 0.236$\pm$0.019 & 79.75 & 293.94s/6.63hr \\
          & 8 & 510305 & Diverged & Diverged & Diverged & Diverged \\
        3WLGNN & 3 & 102150 & 0.407$\pm$0.028 & 0.272$\pm$0.037 & 111.25 & 286.23s/8.88hr  \\
        3WLGNN-E & 3 & 103098 & \good{0.256$\pm$0.054} & 0.140$\pm$0.044 & 117.25 & 334.69s/10.90hr \\
         & 3 & 507603 & 0.303$\pm$0.068 & 0.173$\pm$0.041 & 120.25 & 329.49s/11.08hr \\
         & 8 & 582824 & 0.303$\pm$0.057 & 0.246$\pm$0.043 & 52.50 & 811.27s/12.15hr \\
        \bottomrule
    \end{tabular}
    }
    \label{tab:results}
\end{table}


==> tables.tex <==
\begin{table}
\centering
\makebox[0pt][c]{\parbox{1.0\textwidth}{%
    \begin{minipage}[!t]{0.49\hsize}\centering
        \caption{%ZINC: Study of GNN 
        Performance on ZINC (lower is better). Results are averaged over 4 runs with 4 different seeds. \best{Red}: the best model and \good{Violet}: good models. 
    }
    \vspace{3pt}
    \scalebox{0.43}{
    % \begin{tabular}{r|c|c|c|c|c|c}
    % Vijay: following NeurIPS style to not have vertical rules/lines
    \begin{tabular}{rrccccc}
        \toprule
        \textbf{Model} & \textbf{$L$} & \textbf{\#Param} & \textbf{Test MAE$\pm$s.d.} & \textbf{Train MAE$\pm$s.d.} & \textbf{\#Epochs} & \textbf{Epoch/Total} \\
        \midrule
        \midrule
        MLP & 4 & 108975 & 0.706$\pm$0.006 & 0.644$\pm$0.005 & 116.75 & 1.01s/0.03hr \\
        % & 16 & 505225 & 0.711$\pm$0.001 & 0.654$\pm$0.003 & 104.25 & 1.50s/0.04hr \\
        \midrule
        GCN & 4 & 103077 & 0.459$\pm$0.006 & 0.343$\pm$0.011 & 196.25 & 2.89s/0.16hr \\
         & 16 & 505079 & 0.367$\pm$0.011 & 0.128$\pm$0.019 & 197.00 & 12.78s/0.71hr \\
        GraphSage & 4 & 94977 & 0.468$\pm$0.003 & 0.251$\pm$0.004 & 147.25 & 3.74s/0.15hr \\
         & 16 & 505341 & 0.398$\pm$0.002 & 0.081$\pm$0.009 & 145.50 & 16.61s/0.68hr \\
        \midrule
        MoNet & 4 & 106002 & 0.388$\pm$0.008 & 0.295$\pm$0.019 & 154.75 & 12.33s/0.54hr \\
         & 16 & 504013 & 0.294$\pm$0.011 & 0.115$\pm$0.015 & 152.00 & 20.74s/0.88hr \\
        GAT & 4 & 102385 & 0.475$\pm$0.007 & 0.317$\pm$0.006 & 137.50 & 2.93s/0.11hr \\
         & 16 & 531345 & 0.384$\pm$0.007 & 0.067$\pm$0.004 & 144.00 & 12.98s/0.53hr \\
        GatedGCN & 4 & 105735 & 0.435$\pm$0.011 & 0.287$\pm$0.014 & 173.50 & 5.76s/0.28hr \\
        GatedGCN-E & 4 & 105875 & 0.375$\pm$0.003 & 0.236$\pm$0.007 & 194.75 & 5.37s/0.29hr \\
         & 16 & 504309 & \good{0.282$\pm$0.015} & 0.074$\pm$0.016 & 166.75 & 20.50s/0.96hr \\
        GatedGCN-E-PE & 16 & 505011 & \best{0.214$\pm$0.006} & 0.033$\pm$0.012 & 167.00 & 20.74s/0.98hr \\
        \midrule
        GIN & 4 & 103079 & 0.387$\pm$0.015 & 0.319$\pm$0.015 & 153.25 & 2.29s/0.10hr \\
         & 16 & 509549 & 0.526$\pm$0.051 & 0.444$\pm$0.039 & 147.00 & 10.22s/0.42hr \\
        RingGNN & 2 & 97978 & 0.512$\pm$0.023 & 0.383$\pm$0.020 & 90.25 & 327.65s/8.32hr  \\
        RingGNN-E & 2 & 104403 & 0.363$\pm$0.026 & 0.243$\pm$0.025 & 95.00 & 366.29s/9.76hr \\
         & 2 & 527283 & 0.353$\pm$0.019 & 0.236$\pm$0.019 & 79.75 & 293.94s/6.63hr \\
          & 8 & 510305 & diverged* & diverged* & diverged* & diverged* \\
        3WLGNN & 3 & 102150 & 0.407$\pm$0.028 & 0.272$\pm$0.037 & 111.25 & 286.23s/8.88hr  \\
        3WLGNN-E & 3 & 103098 & \good{0.256$\pm$0.054} & 0.140$\pm$0.044 & 117.25 & 334.69s/10.90hr \\
         & 3 & 507603 & 0.303$\pm$0.068 & 0.173$\pm$0.041 & 120.25 & 329.49s/11.08hr \\
         & 8 & 582824 & 0.303$\pm$0.057 & 0.246$\pm$0.043 & 52.50 & 811.27s/12.15hr \\
        \bottomrule
    \vspace{-0.25cm}\\
   \multicolumn{7}{l}{\scalebox{1}{
  \scriptsize{\textit{GNN-E are models using bond types as input edge features.}}
  }} \\
   \multicolumn{7}{l}{\scalebox{1}{
  \scriptsize{\textit{GatedGCN-E-PE uses bond types as input edge features and Laplacian eigenvectors as positional encodings.}}
  }} \\
   \multicolumn{7}{l}{\scalebox{1}{
  \scriptsize{\textit{RingGNN-E with L8+RC diverged* with inital learning rates of $10^{-3},10^{-4},10^{-5}$.}}
  }} \\
    \end{tabular}
    }
    \label{tab:zinc}
    \end{minipage}
    \hfill
    \begin{minipage}[!t]{0.49\hsize}\centering
        \caption{%TSP: Study of GNN Performance
        Performance on TSP (higher is better). Results are averaged over 4 runs with 4 different seeds. \best{Red}: the best model and \good{Violet}: good models. 
        }
    \vspace{3pt}
    \scalebox{0.44}{
    % \begin{tabular}{r|c|c|c|c|c|c}
    \begin{tabular}{rrccccc}
        \toprule
        \textbf{Model} & \textbf{$L$} & \textbf{\#Param} & \textbf{Test F1$\pm$s.d.} & \textbf{Train F1$\pm$s.d.} & \textbf{\#Epochs} & \textbf{Epoch/Total} \\
        \midrule
        \midrule
        MLP & 4 & 96956 & 0.544$\pm$0.001 & 0.544$\pm$0.001 & 164.25 & 50.15s/2.31hr \\
        \midrule
        GCN & 4 & 95702 & 0.630$\pm$0.001 & 0.631$\pm$0.001 & 261.00 & 152.89s/11.15hr \\
        GraphSage & 4 & 99263 & 0.665$\pm$0.003 & 0.669$\pm$0.003 & 266.00 & 157.26s/11.68hr \\
        \midrule
        MoNet & 4 & 99007 & 0.561$\pm$0.018 & 0.561$\pm$0.018 & 27.50 & 1573.25s/12.66hr \\
        GAT & 4 & 96182 & 0.671$\pm$0.002 & 0.673$\pm$0.002 & 328.25 & 68.23s/6.25hr \\
        GatedGCN & 4 & 97858 & \good{0.791$\pm$0.003} & 0.793$\pm$0.003 & 159.00 & 218.20s/9.72hr \\
        GatedGCN-E & 4 & 97858 & \good{0.808$\pm$0.003} & 0.811$\pm$0.003 & 197.00 & 218.51s/12.04hr \\
        GatedGCN-E & 16 & 500770 & \best{0.838$\pm$0.002} & 0.850$\pm$0.001 & 53.00 & 807.23s/12.17hr \\
        \midrule
        GIN & 4 & 99002 & 0.656$\pm$0.003 & 0.660$\pm$0.003 & 273.50 & 72.73s/5.56hr \\
        RingGNN & 2 & 106862 & 0.643$\pm$0.024 & 0.644$\pm$0.024 & 2.00 & 17850.52s/17.19hr\\
        & 2 & 507938 & 0.704$\pm$0.003 & 0.705$\pm$0.003 & 3.00 & 12835.53s/16.08hr \\
        & 8 & 506564 & diverged* & diverged* & diverged* & diverged*\\
        3WLGNN & 3 & 106366 & 0.694$\pm$0.073 & 0.695$\pm$0.073 & 2.00 & 17468.81s/16.59hr\\
        &3 & 506681 & 0.288$\pm$0.311 & 0.290$\pm$0.312 & 2.00 & 17190.17s/16.51hr\\
        % & 3 & 503964 & 0.000$\pm$0.000 & 0.000$\pm$0.000 & 1.00 & 30809.80s/21.18hr \\
        & 8 & 508832 & OOM & OOM & OOM & OOM\\
        \midrule
        \multicolumn{3}{c}{$k$-NN Heuristic, $k=2$ \quad :} & \multicolumn{4}{l}{Test F1: 0.693} \\
        \bottomrule
    \vspace{-0.25cm}\\
   \multicolumn{7}{l}{\scalebox{1}{
  \scriptsize{\textit{GatedGCN-E use the Euclidean distance between nodes as input edge features.}}
  }} \\
   \multicolumn{7}{l}{\scalebox{1}{
  \scriptsize{\textit{RingGNN with L8+RC diverged* with inital learning rates of $10^{-3},10^{-4},10^{-5}$.}}
  }} \\
   \multicolumn{7}{l}{\scalebox{1}{
  \scriptsize{\textit{RingGNN/3WLGNN with L2/L3 and 100k parameters achieved 0.733$\pm$0.020/0.649$\pm$0.051 resp. on the test set after training for 48hr. }}
  }} \\
    \end{tabular}
    }
    \label{tab:tsp}
%   \scalebox{0.55}{
%   \vijay{Vijay: We can fill this space with some common meta info later about all tables.
% % \vijay{Vijay: Maybe we can remove MLP L16 from ZINC table as well?}
%   }}
    \end{minipage}%
}}
\end{table}


\begin{table}[t]
    \centering
    \caption{%SBMs: Study of GNN Performance.
    Performance on PATTERN and CLUSTER SBM graphs. Accuracy is the mean of the number of nodes correctly classified w.r.t. the class size (higher is better). Results are averaged over 4 runs with 4 different seeds. \best{Red}: the best model, \good{Violet}: good models. 
    % \\ \vijay{Vijay: If this style of arranging two tables looks good to you, we can do the same for MNIST/CIFAR10 as well? And ZINC/TSP also we can bring in half page by putting ZINC on left part and TSP on right part. Doing so, all tables' font size would be similar as seen in this table. } \\ \xb{XB: Yes, this is nice!}
    }
    \vspace{3pt}
    \scalebox{0.52}{
    % Vijay: following NeurIPS style to not have vertical rules/lines
    % \begin{tabular}{c|r|c|c|c|c|c|c}
    \begin{tabular}{rr|ccccc|ccccc}
        \toprule
        & & \multicolumn{5}{c|}{\textbf{PATTERN}} & \multicolumn{5}{c}{\textbf{CLUSTER}}\\
        % \textbf{Dataset} &
        \textbf{Model} & \textbf{$L$} & \textbf{\#Param} & \textbf{Test Acc.$\pm$s.d.} & \textbf{Train Acc.$\pm$s.d.} & \textbf{\#Epochs} & \textbf{Epoch/Total} & \textbf{\#Param} & \textbf{Test Acc.$\pm$s.d.} & \textbf{Train Acc.$\pm$s.d.} & \textbf{\#Epochs} & \textbf{Epoch/Total} \\
        \midrule
        \midrule
        MLP & 4 & 105263 & 50.519$\pm$0.000 & 50.487$\pm$0.014 & 42.25 & 8.95s/0.11hr & 106015 & 20.973$\pm$0.004 & 20.938$\pm$0.002 & 42.25 & 5.83s/0.07hr\\
        %& 16 & & & & & & 507691 & 20.973$\pm$0.004 & 20.939$\pm$0.003 & 61.50 & 7.18s/0.13hr\\
        \cline{1-12}
        GCN & 4 & 100923 & 63.880$\pm$0.074 & 65.126$\pm$0.135 & 105.00 & 118.85s/3.51hr & 101655 & 53.445$\pm$2.029 & 54.041$\pm$2.197 & 70.00 & 65.72s/1.30hr\\
        & 16 & 500823 & 71.892$\pm$0.334 & 78.409$\pm$1.592 & 81.50 & 492.19s/11.31hr & 501687 & 68.498$\pm$0.976 & 71.729$\pm$2.212 & 79.75 & 270.28s/6.08hr\\
        GraphSage & 4 & 101739 & 50.516$\pm$0.001 & 50.473$\pm$0.014 & 43.75 & 93.41s/1.17hr & 102187 & 50.454$\pm$0.145 & 54.374$\pm$0.203 & 64.00 & 53.56s/0.97hr\\
        & 16 & 502842 & 50.492$\pm$0.001 & 50.487$\pm$0.005 & 46.50 & 391.19s/5.19hr & 503350 & 63.844$\pm$0.110 & 86.710$\pm$0.167 & 57.75 & 225.61s/3.70hr\\
        \cline{1-12}
        MoNet & 4 & 103775 & {85.287$\pm$0.113} & 85.304$\pm$0.134 & 43.00 & 996.95s/12.41hr & 104227 & 57.508$\pm$0.660 & 57.826$\pm$0.693 & 63.75 & 692.79s/12.18hr\\
        & 16 & 511487 & \good{85.417$\pm$0.203} & 85.483$\pm$0.193 & 40.00 & 1068.77s/12.37hr & 511999 & 65.830$\pm$1.108 & 66.996$\pm$1.152 & 66.00 & 652.34s/12.28hr\\
        GAT & 4 & 109936 & 75.824$\pm$1.823 & 77.883$\pm$1.632 & 96.00 & 20.92s/0.57hr & 110700 & 57.732$\pm$0.323 & 58.331$\pm$0.342 & 67.25 & 14.17s/0.27hr\\
        & 16 & 526990 & 78.271$\pm$0.186 & 90.212$\pm$0.476 & 53.50 & 50.33s/0.77hr & 527874 & \good{70.587$\pm$0.447} & 76.074$\pm$1.362 & 73.50 & 35.94s/0.75hr\\
        GatedGCN & 4 & 104003 & 84.480$\pm$0.122 & 84.474$\pm$0.155 & 78.75 & 139.01s/3.09hr & 104355 & 60.404$\pm$0.419 & 61.618$\pm$0.536 & 94.50 & 79.97s/2.13hr\\
        & 16 & 502223 & \good{85.568$\pm$0.088} & 86.007$\pm$0.123 & 65.25 & 644.71s/11.91hr & 502615 & \best{73.840$\pm$0.326} & 87.880$\pm$0.908 & 60.00 & 400.07s/6.81hr\\
        GatedGCN-PE & 16 & 505421 & \best{86.363$\pm$0.127} & 86.810$\pm$0.126 & 60.00 & 647.95s/11.09hr & 503473 & \best{74.088$\pm$0.344} & 90.252$\pm$1.048 & 56.50 & 400.34s/6.45hr \\
        %& GatedGCN-E \\
        \cline{1-12}
        GIN & 4 & 100884 & \good{85.590$\pm$0.011} & 85.852$\pm$0.030 & 93.00 & 15.24s/0.40hr & 103544 & 58.384$\pm$0.236 & 59.480$\pm$0.337 & 74.75 & 10.71s/0.23hr\\
        & 16 & 508574 & 85.387$\pm$0.136 & 85.664$\pm$0.116 & 86.75 & 25.14s/0.62hr & 517570 & 64.716$\pm$1.553 & 65.973$\pm$1.816 & 80.75 & 20.67s/0.47hr\\
        RingGNN & 2 & 105206 & \good{86.245$\pm$0.013} & 86.118$\pm$0.034 & 75.00 & 573.37s/12.17hr & 104746 & 42.418$\pm$20.063 & 42.520$\pm$20.212 & 74.50 & 428.24s/8.79hr\\
        & 2 & 504766 & \good{86.244$\pm$0.025} & 86.105$\pm$0.021 & 72.00 & 595.97s/12.15hr & 524202 & 22.340$\pm$0.000 & 22.304$\pm$0.000 & 43.25 & 501.84s/6.22hr\\
        & 8 & 505749 & \textrm{diverged*} & \textrm{diverged*} & \textrm{diverged*} & \textrm{diverged*} & 514380 & \textrm{diverged*} & \textrm{diverged*} & \textrm{diverged*} & \textrm{diverged*}\\
        3WLGNN & 3 & 103572 & \good{85.661$\pm$0.353} & 85.608$\pm$0.337 & 95.00 & 304.79s/7.88hr & 105552 & 57.130$\pm$6.539 & 57.404$\pm$6.597 & 116.00 & 219.51s/6.52hr\\
        & 3 & 502872 & \good{85.341$\pm$0.207} & 85.270$\pm$0.198 & 81.75 & 424.23s/9.56hr & 507252 & 55.489$\pm$7.863 & 55.736$\pm$8.024 & 66.00 & 319.98s/5.79hr \\
        & 8 & 581716 & \textrm{diverged*} & \textrm{diverged*} & \textrm{diverged*} & \textrm{diverged*} & 586788 & \textrm{diverged*} & \textrm{diverged*} & \textrm{diverged*} & \textrm{diverged*}\\
        % \midrule
        % CLUSTER FROM HERE ###############################
        % \parbox[t]{2mm}{\multirow{19}{*}{\rotatebox[origin=c]{90}{CLUSTER}}} 
        % & MLP & 4 & 106015 & 20.973$\pm$0.004 & 20.938$\pm$0.002 & 42.25 & 5.83s/0.07hr \\
        % &  & 16 & 507691 & 20.973$\pm$0.004 & 20.939$\pm$0.003 & 61.50 & 7.18s/0.13hr \\
        % \cline{2-8}
        % & GCN & 4 & 101655 & 53.445$\pm$2.029 & 54.041$\pm$2.197 & 70.00 & 65.72s/1.30hr \\
        % & & 16 & 501687 & 68.498$\pm$0.976 & 71.729$\pm$2.212 & 79.75 & 270.28s/6.08hr \\
        % & GraphSage & 4 & 102187 & 50.454$\pm$0.145 & 54.374$\pm$0.203 & 64.00 & 53.56s/0.97hr \\
        % & & 16 & 503350 & 63.844$\pm$0.110 & 86.710$\pm$0.167 & 57.75 & 225.61s/3.70hr \\
        % \cline{2-8}
        % & MoNet & 4 & 104227 & 57.508$\pm$0.660 & 57.826$\pm$0.693 & 63.75 & 692.79s/12.18hr \\
        % & & 16 & 511999 & 65.830$\pm$1.108 & 66.996$\pm$1.152 & 66.00 & 652.34s/12.28hr \\
        % & GAT & 4 & 110700 & 57.732$\pm$0.323 & 58.331$\pm$0.342 & 67.25 & 14.17s/0.27hr \\
        % & & 16 & 527874 & \good{70.587$\pm$0.447} & 76.074$\pm$1.362 & 73.50 & 35.94s/0.75hr \\
        % & GatedGCN & 4 & 104355 & 60.404$\pm$0.419 & 61.618$\pm$0.536 & 94.50 & 79.97s/2.13hr \\
        % %& GatedGCN & 32 & 807995 & 74.636$\pm$0.390 & 90.796$\pm$0.986 & 54.00 & 753.95s/11.59hr \\
        % &  & 16 & 502615 & \best{73.840$\pm$0.326} & 87.880$\pm$0.908 & 60.00 & 400.07s/6.81hr \\
        %& GatedGCN-E \\
        % \cline{2-8}
        % & GIN & 4 & 103544 & 58.384$\pm$0.236 & 59.480$\pm$0.337 & 74.75 & 10.71s/0.23hr \\
        % &  & 16 & 517570 & 64.716$\pm$1.553 & 65.973$\pm$1.816 & 80.75 & 20.67s/0.47hr \\
        % & RingGNN & 2 & 104746 & 42.418$\pm$20.063 & 42.520$\pm$20.212 & 74.50 & 428.24s/8.79hr \\
        % &  & 2 & 524202 & 22.340$\pm$0.000 & 22.304$\pm$0.000 & 43.25 & 501.84s/6.22hr \\
        % & & 8 & 514380 & \textrm{diverged} & \textrm{diverged} & \textrm{diverged} & \textrm{diverged} \\
        % & 3WLGNN & 3 & 105552 & 57.130$\pm$6.539 & 57.404$\pm$6.597 & 116.00 & 219.51s/6.52hr \\
        % &  & 3 & 507252 & 55.489$\pm$7.863 & 55.736$\pm$8.024 & 66.00 & 319.98s/5.79hr \\
        % & & 8 & 586788 & \textrm{diverged} & \textrm{diverged} & \textrm{diverged} & \textrm{diverged} \\
        \bottomrule
    \vspace{-0.25cm}\\
   \multicolumn{12}{l}{\scalebox{1}{
  \scriptsize{\textit{GatedGCN-PE uses Laplacian eigenvectors as positional encodings.}}
  }} \\
   \multicolumn{12}{l}{\scalebox{1}{
  \scriptsize{\textit{RingGNN/3WLGNN with L8+RC diverged* with initial learning rates of $10^{-3},10^{-4},10^{-5}$.}}
  }} \\
    \end{tabular}
    }
    \label{tab:sbms}
\end{table}


\begin{table}[!t]
    \centering
    \caption{%Superpixels: Study of GNN Performance. 
    Performance on MNIST and CIFAR10 superpixel graphs. Accuracy is the number of nodes correctly classified (higher is better). Results are averaged over 4 runs with 4 different seeds. \best{Red}: the best model, \good{Violet}: good models.
    % \textit{Models with * have not converged in 12 hrs.} %\vijay{Vijay: Lets remove GatedGCN-E from both MNIST and CIFAR10; no significant gain compared to GatedGCN; besides we have not used the -E variants for WLGNNs.} % XB: Agree
    % Note to write in expts: RingGNN use init\_lr 1e-4, min\_lr 1e-6; others use init\_lr 1e-4, min\_lr 1e-5 \\ 
    }
    \vspace{3pt}
    \scalebox{0.53}{
    % \begin{tabular}{c|r|c|c|c|c|c|c}
    \begin{tabular}{rr|ccccc|ccccc}
        \toprule
        & & \multicolumn{5}{c|}{\textbf{MNIST}} & \multicolumn{5}{c}{\textbf{CIFAR10}}\\
        \textbf{Model} & \textbf{$L$} & \textbf{\#Param} & \textbf{Test Acc.$\pm$s.d.} & \textbf{Train Acc.$\pm$s.d.} & \textbf{\#Epochs} & \textbf{Epoch/Total} & \textbf{\#Param} & \textbf{Test Acc.$\pm$s.d.} & \textbf{Train Acc.$\pm$s.d.} & \textbf{\#Epochs} & \textbf{Epoch/Total} \\
        \midrule
        \midrule
        % \parbox[t]{2mm}{\multirow{10}{*}{\rotatebox[origin=c]{90}{MNIST}}} & 
        MLP & 4 & 104044 & 95.340$\pm$0.138 & 97.432$\pm$0.470 & 232.25 & 22.74s/1.48hr & 104380 & 56.340$\pm$0.181 & 65.113$\pm$1.685 & 185.25 & 29.48s/1.53hr\\
        \cline{1-12}
        GCN & 4 & 101365 & 90.705$\pm$0.218 & 97.196$\pm$0.223 & 127.50 & 83.41s/2.99hr & 101657 & 55.710$\pm$0.381 & 69.523$\pm$1.948 & 142.50 & 109.70s/4.39hr\\
        GraphSage & 4 & 104337 & \best{97.312$\pm$0.097} & 100.000$\pm$0.000 & 98.25 & 113.12s/3.13hr & 104517 & \good{65.767$\pm$0.308} & 99.719$\pm$0.062 & 93.50 & 124.61s/3.29hr\\
        \cline{1-12}
        MoNet & 4 & 104049 & 88.507$\pm$1.414 & 90.895$\pm$1.910 & 57.75 & 750.10s/12.28hr & 104229 & 49.462$\pm$1.386 & 52.671$\pm$1.991 & 42.50 & 1031.36s/12.42hr\\
        GAT & 4 & 110400 & 95.535$\pm$0.205 & 99.994$\pm$0.008 & 104.75 & 42.26s/1.25hr & 110704 & 64.223$\pm$0.455 & 89.114$\pm$0.499 & 103.75 & 55.27s/1.62hr\\
        GatedGCN & 4 & 104217 & \best{97.340$\pm$0.143} & 100.000$\pm$0.000 & 96.25 & 128.79s/3.50hr & 104357 & \best{67.312$\pm$0.311} & 94.553$\pm$1.018 & 97.00 & 154.15s/4.22hr\\
        %& GatedGCN-E & 4 & 104217 & \best{97.350$\pm$0.098} & 100.000$\pm$0.000 & 96.00 & 133.47s/3.61hr \\
        \cline{1-12}
        GIN & 4 & 105434 & \good{96.485$\pm$0.252} & 100.000$\pm$0.000 & 128.00 & 39.22s/1.41hr & 105654 & 55.255$\pm$1.527 & 79.412$\pm$9.700 & 141.50 & 52.12s/2.07hr\\
        RingGNN & 2 & 105398 & 11.350$\pm$0.000 & 11.235$\pm$0.000 & 14.00 & 2945.69s/12.77hr & 105165 & 19.300$\pm$16.108 & 19.556$\pm$16.397 & 13.50 & 3112.96s/13.00hr\\
        & 2 & 505182 & 91.860$\pm$0.449 & 92.169$\pm$0.505 & 16.25 & 2575.99s/12.63hr & 504949 & 39.165$\pm$17.114 & 40.209$\pm$17.790 & 13.75 & 2998.24s/12.60hr \\
        & 8 & 506357 & diverged* & diverged* & diverged* & diverged* & 510439 & diverged* & diverged* & diverged* & diverged*\\
        3WLGNN & 3 & 108024 & 95.075$\pm$0.961 & 95.830$\pm$1.338 & 27.75 & 1523.20s/12.40hr & 108516 & 59.175$\pm$1.593 & 63.751$\pm$2.697 & 28.50 & 1506.29s/12.60hr \\
        & 3 & 501690 & 95.002$\pm$0.419 & 95.692$\pm$0.677 & 26.25 & 1608.73s/12.42hr & 502770 & 58.043$\pm$2.512 & 61.574$\pm$3.575 & 20.00 & 2091.22s/12.55hr\\
        & 8 & 500816 & diverged* & diverged* & diverged* & diverged* & 501584 & diverged* & diverged* & diverged* & diverged* \\
        % \midrule
        % CIFAR10 starts from here ########
        % \parbox[t]{2mm}{\multirow{10}{*}{\rotatebox[origin=c]{90}{CIFAR10}}} & MLP & 4 & 104380 & 56.340$\pm$0.181 & 65.113$\pm$1.685 & 185.25 & 29.48s/1.53hr \\
        % \cline{2-8}
        % & GCN & 4 & 101657 & 55.710$\pm$0.381 & 69.523$\pm$1.948 & 142.50 & 109.70s/4.39hr \\
        % & GraphSage & 4 & 104517 & \good{65.767$\pm$0.308} & 99.719$\pm$0.062 & 93.50 & 124.61s/3.29hr \\
        % \cline{2-8}
        % & MoNet* & 4 & 104229 & 49.462$\pm$1.386 & 52.671$\pm$1.991 & 42.50* & 1031.36s/12.42hr \\
        % & GAT & 4 & 110704 & 64.223$\pm$0.455 & 89.114$\pm$0.499 & 103.75 & 55.27s/1.62hr \\
        % & GatedGCN & 4 & 104357 & \best{67.312$\pm$0.311} & 94.553$\pm$1.018 & 97.00 & 154.15s/4.22hr \\
        %& GatedGCN-E & 4 & 104357 & \best{67.950$\pm$0.624} & 95.559$\pm$0.961 & 97.50 & 152.88s/4.20hr \\
        % \cline{2-8}
        % & GIN & 4 & 105654 & 55.255$\pm$1.527 & 79.412$\pm$9.700 & 141.50 & 52.12s/2.07hr \\
        % & RingGNN* & 2 & 105165 & 19.300$\pm$16.108 & 19.556$\pm$16.397 & 13.50* & 3112.96s/13.00hr \\
        % & & 2 & 504949 & 39.165$\pm$17.114 & 40.209$\pm$17.790 & 13.75* & 2998.24s/12.60hr \\
        % & & 8 & 510439 & diverged & diverged & diverged & diverged\\
        % & 3WLGNN* & 3 & 108516 & 59.175$\pm$1.593 & 63.751$\pm$2.697 & 28.50* & 1506.29s/12.60hr \\
        % & & 3 & 502770 & 58.043$\pm$2.512 & 61.574$\pm$3.575 & 20.00* & 2091.22s/12.55hr\\
        % & & 8 & 501584 & diverged & diverged & diverged & diverged\\
        \bottomrule
    \vspace{-0.25cm}\\
   \multicolumn{12}{l}{\scalebox{1}{
  \scriptsize{\textit{RingGNN/3WLGNN with L8+RC diverged* with initial learning rates of $10^{-3},10^{-4},10^{-5}$.}}
  }} \\
    \end{tabular}
    }
    \label{tab:superpixels}
\end{table}




\begin{table}
\centering
\makebox[0pt][c]{\parbox{1.0\textwidth}{%
    \begin{minipage}[!t]{0.42\hsize}\centering
        \caption{%COLLAB: Study of GNN Performance% \xb{XB: I would use the 40k config here bc we set the max\_time to 12h in our experimental setting.}
    Performance on COLLAB OGB graph (higher is better). Results are averaged over 4 runs with 4 different seeds. \best{Red}: the best model, \good{Violet}: good models.
    }
    \vspace{3pt}
    \scalebox{0.40}{
    % \begin{tabular}{r|c|c|c|c|c|c}
    \begin{tabular}{rrccccc}
        \toprule
        % \textbf{Model} & \textbf{$L$} & \textbf{\#Param} & \textbf{Test Hits@50.$\pm$s.d.} & \textbf{Train Hits@50.$\pm$s.d.} & \textbf{\#Epochs} & \textbf{Epoch/Total} \\
        \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{$L$}} & \multirow{2}{*}{\textbf{\#Par.}} & \textbf{Test} & \textbf{Train} & \multirow{2}{*}{\textbf{\#Eps}} & \textbf{Epoch/} \\
         & & & \textbf{Hits@50} & \textbf{Hits@50} & & \textbf{Total} \\
        % \midrule
        % \midrule
        % MLP & 3 & 27625 & 20.989$\pm$2.294 & 32.756$\pm$4.430 & 161.75 & 2.12s/0.10hr \\
        % \midrule
        % GCN & 3 & 26623 & \good{49.261$\pm$0.756} & 90.444$\pm$0.127 & 144.50 & 287.47s/11.62hr \\
        % GraphSage & 3 & 26293 & \good{50.908$\pm$1.122} & 98.617$\pm$1.763 & 157.75 & 241.49s/10.62hr \\
        % \midrule
        % MoNet & 3 & 27316 & 34.548$\pm$3.615 & 57.887$\pm$5.793 & 160.75 & 25.80s/1.17hr \\
        % GAT & 3 & 28561 & \good{50.662$\pm$0.687} & 96.085$\pm$0.499 & 174.50 & 403.52s/19.69hr \\
        % GatedGCN & 3 & 27055 & \best{51.537$\pm$1.038} & 96.524$\pm$1.704 & 188.67 & 376.67s/19.85hr \\
        % GatedGCN-E & 3 & 27055 & 47.212$\pm$2.016 & 85.801$\pm$0.984 & 156.67 & 377.04s/16.49hr \\
        % \midrule
        % GIN & 3 & 26740 & 41.884$\pm$2.467 & 72.370$\pm$4.420 & 160.50 & 7.26s/0.33hr \\
        % \midrule
        % % \multicolumn{2}{c|}{256$\times$235868}
        % Matrix Fact. & 0 & 60546561 & 44.206$\pm$0.452 & 100.000$\pm$0.000 & 254.33 & 2.66s/0.21hr \\
        \midrule
        \midrule
        MLP & 3 & 39441 & 20.350$\pm$2.168 & 29.807$\pm$3.360 & 147.50 & 2.09s/0.09hr \\
        GCN & 3 & 40479 & \good{50.422$\pm$1.131} & 92.112$\pm$0.991 & 122.50 & 351.05s/12.04hr \\
        GraphSage & 3 & 39856 & \good{51.618$\pm$0.690} & 99.949$\pm$0.052 & 152.75 & 277.93s/11.87hr \\
        \midrule
        MoNet & 3 & 39751 & 36.144$\pm$2.191 & 61.156$\pm$3.973 & 167.50 & 26.69s/1.26hr \\
        GAT & 3 & 42637 & \good{51.501$\pm$0.962} & 97.851$\pm$1.114 & 157.00 & 18.12s/0.80hr \\
        GatedGCN & 3 & 40965 & \best{52.816$\pm$1.303} & 96.537$\pm$1.614 & 95.00 & 451.92s/12.05hr \\
        GatedGCN-E & 3 & 40965 & 49.212$\pm$1.560 & 88.747$\pm$1.058 & 95.00 & 451.21s/12.03hr \\
        GatedGCN-PE & 3 & 42769 & \good{52.018$\pm$1.178} & 96.208$\pm$1.833 & 94.50 & 452.34s/12.05hr \\
        \midrule
        GIN & 3 & 39544 & 41.730$\pm$2.284 & 70.555$\pm$4.444 & 140.25 & 8.66s/0.34hr \\
        RingGNN & 2 & 40K & OOM & OOM & OOM & OOM \\
        3WLGNN & 3 & 40K & OOM & OOM & OOM & OOM \\
        \midrule
        % \multicolumn{2}{c|}{256$\times$235868}
        Matrix Fact. & 0 & 60546561 & 44.206$\pm$0.452 & 100.000$\pm$0.000 & 254.33 & 2.66s/0.21hr \\
        \bottomrule
    \vspace{-0.25cm}\\
   \multicolumn{7}{l}{\scalebox{1}{
  \scriptsize{\textit{GatedGCN-E uses collaboration frequency between authors and year of collaboration as input edge features.}}
  }} \\
   \multicolumn{7}{l}{\scalebox{1}{
  \scriptsize{\textit{GatedGCN-PE uses Laplacian eigenvectors as positional encodings.}}
  }} \\
    \end{tabular}
    }
    \label{tab:collab} 
    \end{minipage}
    \hfill
    \begin{minipage}[!t]{0.56\hsize}\centering
        \caption{Study of GNNs with CSL (higher is better). The results are from 5-fold CV, 
        % experiments 
        run 20 times with different seeds. \best{Red}: the best model, \good{Violet}: good models.
    }
    \vspace{5pt}
    \scalebox{0.38}{
    % \begin{tabular}{r|c|c|c|c|c|c|c|c|c|c}
    \begin{tabular}{rcccccccccc}
        \toprule
        %\cline{1-11}
        \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{$L$}} & \multirow{2}{*}{\textbf{\#Param}} & \multicolumn{3}{c|}{\textbf{Test Accuracy}} & \multicolumn{3}{c}{\textbf{Train Accuracy}} & \multirow{2}{*}{\textbf{\#Epochs}} & \multirow{2}{*}{\textbf{Epoch/Total}}  \\
        \cline{4-9}
                & & & \textbf{Mean$\pm$s.d.} & \textbf{Max} & \textbf{Min} & \textbf{Mean$\pm$s.d.} & \textbf{Max} & \textbf{Min} & & \\ 
        % \cline{1-11}
        \midrule
        \midrule
                & & \multicolumn{9}{c}{\textbf{Node positional encoding with Laplacian eigenmaps }} \\
        \cline{3-11}
        MLP & 4 & 101235 & 22.567$\pm$6.089 & 46.667 & 10.000 & 30.389$\pm$5.712 & 43.333 & 10.000 & 109.39 & 0.16s/0.03hr \\
        \midrule
        GCN & 4 & 103847 & \best{100.000$\pm$0.000} & 100.000 & 100.000 & 100.000$\pm$0.000 & 100.000 & 100.000 & 125.64 & 0.40s/0.07hr \\
        GraphSage & 4 & 105867 & \good{99.933$\pm$0.467} & 100.000 & 96.667 & 100.000$\pm$0.000 & 100.000 & 100.000 & 155.00 & 0.50s/0.11hr \\
        \midrule
        MoNet & 4 & 105579 & \good{99.967$\pm$0.332} & 100.000 & 96.667 & 100.000$\pm$0.000 & 100.000 & 100.000 & 130.90 & 0.84s/0.16hr  \\
        GAT & 4 & 101710 & \good{99.933$\pm$0.467} & 100.000 & 96.667 & 100.000$\pm$0.000 & 100.000 & 100.000 & 133.18 & 0.61s/0.12hr  \\
        GatedGCN & 4 & 105407 & \good{99.600$\pm$1.083} & 100.000 & 96.667 & 100.000$\pm$0.000 & 100.000 & 100.000 & 147.06 & 0.66s/0.14hr \\
        \midrule
        GIN & 4 & 107304 & \good{99.333$\pm$1.333} & 100.000 & 96.667 & 100.000$\pm$0.000 & 100.000 & 100.000 & 62.98 & 0.44s/0.04hr  \\
        RingGNN & 2 & 102726 & 17.233$\pm$6.326 & 40.000 & 10.000 & 26.122$\pm$14.382 & 58.889 & 10.000 & 122.75 & 2.93s/0.50hr \\
        & 2 & 505086 & 25.167$\pm$7.399 & 46.667 & 10.000 & 54.533$\pm$18.415 & 82.222 & 10.000 & 120.58 & 3.11s/0.51hr \\
        3WLGNN & 3 & 102054 & 30.533$\pm$9.863 & 56.667 & 10.000 & 99.644$\pm$1.684 & 100.000 & 88.889 & 74.66 & 2.33s/0.25hr   \\
        & 3 & 505347 & 30.500$\pm$8.197 & 56.667 & 13.333 & 100.000$\pm$0.000 & 100.000 & 100.000 & 66.64 & 2.38s/0.23hr \\
        \cline{3-11}
        & & \multicolumn{9}{c}{\textbf{No node positional encoding}} \\
        \cline{3-11}
        All MP-GNNs & 4 & 100K & 10.000$\pm$0.000 & 10.000 & 10.000 & 10.000$\pm$0.000 & 10.000 & 10.000 & - & - \\
        RingGNN & 2 & 101138 & 10.000$\pm$0.000 & 10.000 & 10.000 & 10.000$\pm$0.000 & 10.000 & 10.000 & 103.23 & 3.09s/0.45hr \\
        & 2 & 505325 & 10.000$\pm$0.000 & 10.000 & 10.000 & 10.000$\pm$0.000 & 10.000 & 10.000 & 90.04 & 3.28s/0.42hr \\
        3WLGNN & 3 & 102510 & 95.700$\pm$14.850 & 100.000 & 30.000 & 95.700$\pm$14.850 & 100.000 & 30.000 & 475.81 & 2.29s/1.51hr  \\
        & 3 & 506106 & 97.800$\pm$10.916 & 100.000 & 30.000 & 97.800$\pm$10.916 & 100.000 & 30.000 & 283.80 & 2.28s/0.90hr \\
        \bottomrule
    \end{tabular}
    }
    \label{tab:csl}
    \end{minipage}%
}}
\end{table}







% \begin{table}[!t]
%     \centering
%     \caption{%COLLAB: Study of GNN Performance% \xb{XB: I would use the 40k config here bc we set the max\_time to 12h in our experimental setting.}
%     Performance on COLLAB OGB graph (higher is better). Results are averaged over 4 runs with 4 different seeds. Red: the best model, Violet: good models.
%     }
%     \vspace{3pt}
%     \scalebox{0.50}{
%     % \begin{tabular}{r|c|c|c|c|c|c}
%     \begin{tabular}{rcccccc}
%         \toprule
%         \textbf{Model} & \textbf{$L$} & \textbf{\#Param} & \textbf{Test Hits@50.$\pm$s.d.} & \textbf{Train Hits@50.$\pm$s.d.} & \textbf{\#Epochs} & \textbf{Epoch/Total} \\
%         % \midrule
%         % \midrule
%         % MLP & 3 & 27625 & 20.989$\pm$2.294 & 32.756$\pm$4.430 & 161.75 & 2.12s/0.10hr \\
%         % \midrule
%         % GCN & 3 & 26623 & \good{49.261$\pm$0.756} & 90.444$\pm$0.127 & 144.50 & 287.47s/11.62hr \\
%         % GraphSage & 3 & 26293 & \good{50.908$\pm$1.122} & 98.617$\pm$1.763 & 157.75 & 241.49s/10.62hr \\
%         % \midrule
%         % MoNet & 3 & 27316 & 34.548$\pm$3.615 & 57.887$\pm$5.793 & 160.75 & 25.80s/1.17hr \\
%         % GAT & 3 & 28561 & \good{50.662$\pm$0.687} & 96.085$\pm$0.499 & 174.50 & 403.52s/19.69hr \\
%         % GatedGCN & 3 & 27055 & \best{51.537$\pm$1.038} & 96.524$\pm$1.704 & 188.67 & 376.67s/19.85hr \\
%         % GatedGCN-E & 3 & 27055 & 47.212$\pm$2.016 & 85.801$\pm$0.984 & 156.67 & 377.04s/16.49hr \\
%         % \midrule
%         % GIN & 3 & 26740 & 41.884$\pm$2.467 & 72.370$\pm$4.420 & 160.50 & 7.26s/0.33hr \\
%         % \midrule
%         % % \multicolumn{2}{c|}{256$\times$235868}
%         % Matrix Fact. & 0 & 60546561 & 44.206$\pm$0.452 & 100.000$\pm$0.000 & 254.33 & 2.66s/0.21hr \\
%         \midrule
%         \midrule
%         MLP & 3 & 39441 & 20.350$\pm$2.168 & 29.807$\pm$3.360 & 147.50 & 2.09s/0.09hr \\
%         GCN & 3 & 40479 & \good{50.422$\pm$1.131} & 92.112$\pm$0.991 & 122.50 & 351.05s/12.04hr \\
%         GraphSage & 3 & 39856 & \good{51.618$\pm$0.690} & 99.949$\pm$0.052 & 152.75 & 277.93s/11.87hr \\
%         \midrule
%         MoNet & 3 & 39751 & 36.144$\pm$2.191 & 61.156$\pm$3.973 & 167.50 & 26.69s/1.26hr \\
%         GAT & 3 & 42637 & \good{51.501$\pm$0.962} & 97.851$\pm$1.114 & 157.00 & 18.12s/0.80hr \\
%         GatedGCN & 3 & 40965 & \best{52.816$\pm$1.303} & 96.537$\pm$1.614 & 95.00 & 451.92s/12.05hr \\
%         GatedGCN-E & 3 & 40965 & 49.212$\pm$1.560 & 88.747$\pm$1.058 & 95.00 & 451.21s/12.03hr \\
%         GatedGCN-PE &  \\
%         \midrule
%         GIN & 3 & 39544 & 41.730$\pm$2.284 & 70.555$\pm$4.444 & 140.25 & 8.66s/0.34hr \\
%         RingGNN & 2 & 40K & OOM & OOM & OOM & OOM \\
%         3WLGNN & 3 & 40K & OOM & OOM & OOM & OOM \\
%         \midrule
%         % \multicolumn{2}{c|}{256$\times$235868}
%         Matrix Fact. & 0 & 60546561 & 44.206$\pm$0.452 & 100.000$\pm$0.000 & 254.33 & 2.66s/0.21hr \\
%         \bottomrule
%     \end{tabular}
%     }
%     \label{tab:collab} 
% \end{table}





